Attraction-Repulsion Actor-Critic for Continuous Control Reinforcement Learning

Continuous control tasks in reinforcement learning are important because they provide an important framework for learning in high-dimensional state spaces with deceptive rewards, where the agent can easily become trapped into suboptimal solutions. One way to avoid local optima is to use a population of agents to ensure coverage of the policy space, yet learning a population with the "best" coverage is still an open problem. In this work, we present a novel approach to population-based RL in continuous control that leverages properties of normalizing flows to perform attractive and repulsive operations between current members of the population and previously observed policies. Empirical results on the MuJoCo suite demonstrate a high performance gain for our algorithm compared to prior work, including Soft-Actor Critic (SAC).

==> background.tex <==

This section formalizes the RL setting in a Markov decision process (MDP) and reviews the policy optimization approach considered in this paper along with the general NF framework.

\subsection{Markov decision process}

A discrete-time, finite-horizon, MDP~\citep{bellman1957markovian,puterman2014markov}
is described by a state space $\cS$ (either discrete or continuous), an action space $\cA$ (either discrete or continuous), a transition function $\cP:\cS\times \cA \times \cS\mapsto \Real^+$, and a reward function $r:\cS\times \cA\mapsto \Real$.
MDPs are useful for modelling sequential decision-making problems.
On each round $t$, an agent interacting with this MDP observes the current state $s_t\in\cS$, selects an action $a_t\in\cA$, and observes a reward $r(s_t, a_t) \in\Real$ upon transitioning to a new state $s_{t+1}\sim \cP(s_t, a_t)$.
Let $\gamma\in[0,1]$ be a discount factor.
The goal of an agent evolving in a discounted MDP is to learn a policy $\pi:\cS\times\cA\mapsto[0,1]$ such as taking action $a_t\sim\pi(\cdot|s_t)$ would maximize the expected sum of discounted returns, 
\begin{align}
V^\pi(s) = \Esp_\pi \bigg[\sum_{t=0}^\infty \gamma^t r(s_t, a_t) | s_0 = s\bigg].
\end{align}
The corresponding state-action value function can be written as the expected discounted rewards from taking action $a$ in state $s$, that is
\begin{align}
Q_t^\pi(s,a)=\Esp_{\pi}\bigg[\sum_{i=t}^\infty\gamma^{i-t}r(s_i,a_i)|s_t=s,a_t=a\bigg].
\end{align}
We use $\rho_\pi$ to denote the trajectory distribution induced by following policy $\pi$.
If $\cS$ or $\cA$ are vector spaces, action and space vectors are respectively denoted by $\vec{a}$ and $\vec{s}$.


\subsection{Soft actor-critic}
Soft actor-critic~\citep[SAC,][]{sac} is an off-policy actor-critic strategy which improves stability over previous off-policy algorithms, while maintaining low sample complexity characteristic of off-policy methods (as opposed to on-policy~\citep{trpo}, which tend to have high sample-complexity).
SAC finds the information projection of the Boltzmann Q-function onto the set of diagonal Gaussian policies $\Pi$:
\begin{align}
    \pi=\argmin_{\pi'\in \Pi}  \kl\bigg(\pi'(.|\vec{s}_t) \bigg\lVert \frac{\exp{(\frac{1}{\alpha}Q^{\pi_\old}(\vec{s}_t,.))}}{Z^{\pi_\old}(\vec{s}_t)} \bigg),
    \label{eq:sac_pi_loss}
\end{align}
where $\alpha\in (0,1)$ controls the temperature, i.e. the peakiness of the distribution. Equivalently, the optimized objective can be formulated as a maximum entropy RL task:
\begin{align}
     \pi = \argmin_{\pi'\in \Pi} \Esp_{(\vec{s}_t,\vec{a}_t)\sim\rho_\pi}\bigg[r(\vec{s}_t,\vec{a}_t) +\alpha H(\pi'(\cdot|\vec{s}_t))\bigg],
     \label{eq:sac_pi_constraint}
\end{align}
where the entropy of the policy is denoted pointwise as $H(\pi(\cdot|\vec{s}_t))=\Esp_{\pi}[\log\pi]$ for every state $\vec{s}_t$. When $\pi(\cdot|\vec{s}_t)\sim\mathcal{N}(\vec{\mu},\mat{\Sigma})$ for some mean vector $\vec{\mu}$ and covariance matrix $\mat{\Sigma}$ in a fixed-dimensional space, then $H(\pi(\cdot|\vec{s}_t))\propto \log\det(\mat{\Sigma})$.
% When $\mat{\Sigma}$ is diagonal, then the entropy is directly proportional to the sum of log-variances. 
% The task tackled by SAC can hence be re-formulated as maximizing expected discounted rewards while keeping the volume of the policy at a certain level. Doing so keeps exploration active and prevents mode collapse on the highest reward.
The policy $\pi$, critic $Q$, and value function $V$ are optimized according to the following loss functions:
\begin{align}
    \mathcal{L_{\pi}} &= \Esp_{\vec{s}_t\sim \mathcal{B}}[\Esp_{\vec{a}_t\sim\pi}[\alpha \log \pi(\vec{a}_t|\vec{s}_t)-Q(\vec{s}_t,\vec{a}_t)]]
    \nonumber\\
\mathcal{L}_{Q} &= \underset{(s,a,r,s') \sim \mathcal{B}  }{\Esp}\big[(Q(s,a)-(r+\gamma Q(s',\pi(.|s'))))^2\big]
\nonumber\\
    \cL_V &= \Esp_{\vec{s}_t \sim \cD}\bigg[\frac{1}{2}\big\{V_\nu^\pi(\vec{s}_t)  -\Esp_{\vec{a}_t\sim \pi}[Q(\vec{s}_t,\vec{a}_t)-\alpha\log\pi(\vec{a}_t|\vec{s}_t)]\big\}^2\bigg] \label{eq:v_loss}.
\end{align}

\subsection{Normalizing flows}

Normalizing flows~\citep{rezende2015variational} were introduced as a means of transforming simple distributions into more complex distributions using a learnable and invertible function.
Given a random variable $\vec{z}_0$ with density $q_0$, NF introduces a set of differentiable and invertible functions, $\{f_i\}_{i=1}^{N}$, which generate a sequence of $d$-dimensional random variables, $\{\vec{z}_i\}_{i=1}^N$, each with log-density,
\begin{align}
    \log q_j(\vec{z}_j)= \log q_0(\vec{z}_0)- \sum_{i=1}^j\log \Bigl| \text{det} \frac{\partial f_i(\vec{z}_{i-1})}{\partial \vec{z}_{i-1}} \Bigr|.
\end{align}

%
% Specific forms of the mapping can be selected based on desired properties: highly expressive and sometimes invertible maps~\citep{rezende2015variational}, always invertible affine transformations~\citep{iaf}, volume-preserving and orthogonal transformations~\citep{tomczak2016improving} or always invertible and highly expressive networks~\citep{naf}.
% Due to the high time complexity of RL algorithms, it is preferable to maximally reduce the dimensionality of the actor models while keeping the sample complexity on-par. For this reason, we propose to use the highly expressive and yet very light family of radial contractions around a point $\vec{z}_0$, originally introduced by \cite{rezende2015variational} and defined as
%
Because SAC uses explicit, yet simple parametric policies, NFs can be used to transform the SAC policy into a richer one (e.g., multimodal) without risk loss of information.
Here we follow \citet{preprint}, which uses a family of radial contractions around a point $\vec{z}_0\in\Real^d$,
\begin{align}
    f(\vec{z})=\vec{z}+\frac{\beta}{\alpha+||\vec{z}-\vec{z}_0||_2}(\vec{z}-\vec{z}_0)
\end{align}
% with a closed-form determinant
% \begin{align}
%     \Bigl| \det\frac{\partial f(\vec{z})}{\partial\vec{z}}\Bigr|
%     &= [1+\beta h(\alpha,r)]^{d-1} \nonumber \\
%     &\qquad \cdot [1+\beta h(\alpha,r)+\beta h'(\alpha,r)r]
% \end{align}
for $\alpha\in \mathbb{R}^{+}$ and $\beta\in \mathbb{R}$.
% Inspired by [CITE PREPRINT], we make use of highly expressive and light (parameter-wise) radial policies learned through soft actor-critic updates.
This results in a rich set of policies comprised of an initial noise sample $\vec{a}_0$, a state-noise embedding $h_\theta(\vec{a}_0,\vec{s}_t)$, and a NF $\{f_{\phi_i}\}_{i=1}^N$ of arbitrary length $N$, parametrized by $\phi=\{\vec{\phi}_i\}_{i=1}^N$. Sampling from the policy $\pi_{\phi,\theta}(\vec{a}_t|\vec{s}_t)$ can be described by the following set of equations:
\begin{align}
\label{eq:sac_nf}
    \vec{a}_0 &\sim \mathcal{N}(0,\mat{I});
        \quad
    \vec{z} = h_\theta(\vec{a}_0,\vec{s}_t);
    \quad
    \vec{a}_t = f_{\phi_{N}} \circ f_{\phi_{N-1}} \circ...  \circ f_{\phi_{1}} (\vec{z}),
\end{align}
where $h_{\theta}=\vec{a}_0 \vec{\sigma}\mat{I} + \mu(\vec{s}_t)$ depends on the state and the noise variance $\sigma>0$, for which the later can be taken conditional $\sigma(\vec{s})$, or average $\sigma$.\rdh{I don't understand this statement}.
\rdh{Also I don't think we should go into normalizing flows in too much detail. It doesn't seem to be that important other than it's a way to make the policy a little more rich. We just rely on some paper (ours that got rejected) that noone has heard about. There aren't even experiments that show that NF helps!}
\audrey{It may be a good idea to state explictely what is optimized in SAC-NF (can refer to Eq.3, 4, 5 if relevant). We cannot expect people to go read the SAC-NF preprint in order to understand this work.}\bogdan{corrected}

\rdh{Why isn't evolutionary algorithms A/R background? Eqs 9, 10 should probably be here!}
